Heteroscedastic Uncertainty Estimation Framework for Unsupervised Registration

Deep learning methods for unsupervised registration often rely on objectives that assume a uniform noise level across the spatial domain (e.g. mean-squared error loss), but noise distributions are often heteroscedastic and input-dependent in real-world medical images. Thus, this assumption often leads to degradation in registration performance, mainly due to the undesired influence of noise-induced outliers. To mitigate this, we propose a framework for heteroscedastic image uncertainty estimation that can adaptively reduce the influence of regions with high uncertainty during unsupervised registration. The framework consists of a collaborative training strategy for the displacement and variance estimators, and a novel image fidelity weighting scheme utilizing signal-to-noise ratios. Our approach prevents the model from being driven away by spurious gradients caused by the simplified homoscedastic assumption, leading to more accurate displacement estimation. To illustrate its versatility and effectiveness, we tested our framework on two representative registration architectures across three medical image datasets. Our method consistently outperforms baselines and produces sensible uncertainty estimates. The code is publicly available at \url{https://voldemort108x.github.io/hetero_uncertainty/}.

==> tables/sigma_z_table.tex <==
\begin{table}[tb] 
    \centering
    \begin{adjustbox}{scale=0.68}
    \begin{tabular}{lcccccccc}
    \toprule
        & \multicolumn{2}{c}{Uncertainty} & \multicolumn{3}{c}{ACDC \cite{bernard_deep_2018}} & \multicolumn{3}{c}{CAMUS \cite{leclerc_deep_2019}}  \\
    \cmidrule(lr){2-3}  \cmidrule(lr){4-6} \cmidrule(lr){7-9} 
        & $\sigma_z^2$ & $\sigma_I^2$  & DSC $\uparrow$ & HD $\downarrow$ & ASD $\downarrow$ & DSC $\uparrow$ & HD $\downarrow$ & ASD $\downarrow$  \\\midrule 
        %\multicolumn{12}{c}{Gaussian additive noise assumption $p()$}\\
    \midrule
        Vxm \cite{balakrishnan_voxelmorph_2019}   & \xmark &\xmark  & 80.20 & 4.64 & 1.24 & 81.76 & 8.93 & 1.70  \\\midrule
        Vxm-diff \cite{dalca_unsupervised_2019}   & \cmark & \xmark & 76.19 & 5.75 & \textbf{1.19} & 76.74 & 10.76 & 1.88  \\
        Ours         & \cmark & \xmark & 79.80 & 4.74 & 1.22 & 81.47 &  8.67 & 1.69  \\\midrule
        Ours         & \xmark & \cmark & \textbf{80.73} & \textbf{4.57} & 1.21 & \textbf{81.96} & 8.80 & 1.66  \\
        Ours         & \cmark & \cmark & 79.87 & 4.62 & 1.20 & 81.91 & \textbf{8.54} & \textbf{1.65}  \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Our method raises the upper bound on registration accuracy while providing useful displacement uncertainty estimates $\hat{\sigma}_z$.}
    \label{tab:sigma_z}
\end{table}
